Regularity of minimizing $p$-harmonic maps into spheres and sharp Kato inequality

We study regularity of minimizing $p$-harmonic maps $u \colon B^3 \to \mathbb{S}^3$ for $p$ in the interval $[2,3]$. For a long time, regularity was known only for $p = 3$ (essentially due to Morrey) and $p = 2$ (Schoen-Uhlenbeck), but recently Gastel extended the latter result to $p \in [2,2+\frac{2}{15}]$ using a version of Kato inequality. Here, we establish regularity for a small interval $p\in [2.961,3]$ by combining Morrey's methods with Hardt and Lin's Extension Theorem. We also improve on the other result by obtaining regularity for $p \in [2,p_0]$ with $p_0 = \frac{3+\sqrt{3}}{2} \approx 2.366$. In relation to this, we address a question posed by Gastel and prove a sharp Kato inequality for $p$-harmonic maps in two-dimensional domains, which is of independent interest.

==> macros.tex <==
\usepackage{tikz}
%\usepackage{pgf,tikz,pgfplots} %For TikZ % MM: ale czy potrzebujemy coś poza tikzem?
%\pgfplotsset{compat=1.14}		% MM: czy to jest potrzebne do jakiejś fajnej czcionki? (tak kiedyś było) Bo u mnie nie działa
%% MM: Jest jeszcze parę pakietów tikzowych, ale chyba ich nie potrzeba
%% For TikZ
%\usetikzlibrary{arrows}
%\usetikzlibrary{calc}
%% For TikZ
%\usetikzlibrary{patterns}
%% For TikZ
%\usepackage{pgfplots}
%\usetikzlibrary{intersections, pgfplots.fillbetween}
%% MM: znowu Tikz   
%%%%%% For TikZ warning
%\pgfdeclarelayer{ft}
%\pgfdeclarelayer{bg}
%\pgfsetlayers{bg,main,ft}
%%%%%%%%%%%TIKZ%%%%%%%%%%%%%%%%%%%%
%\tikzset{>=stealth}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\usepackage{mathrsfs}
%\usepackage{float} %for figure H option
% \usepackage[notcite,notref]{showkeys} 
\usepackage[colorlinks=true,urlcolor=blue, citecolor=red,linkcolor=blue,linktocpage,pdfpagelabels, bookmarksnumbered,bookmarksopen]{hyperref}
\usepackage[hyperpageref]{backref}
\usepackage{cleveref}
\usepackage{xcolor}
\usepackage{amsthm} %for citing inside theorem header
\usepackage{latexsym,amsmath,amssymb}
%\usepackage[notref,notcite]{showkeys}
\usepackage{accents}
\usepackage[colorinlistoftodos,prependcaption,textsize=tiny]{todonotes}
% \usepackage{ marvosym } %Has \Heart
\usepackage{a4wide}
\usepackage{soul}
\usepackage{mathtools} %For \chi with a much lower index (\mychi)
\usepackage{xparse} %For a new definiton of \chi with a slightly lower index
\usepackage{enumitem}



%%%%%% colors %%%%%%%
% \definecolor{chameleongreen}{RGB}{98,189,25} %%% for Michal's green
% \definecolor{bluish}{rgb}{0,0,0.8}
% \definecolor{redish}{rgb}{1,0,0}
\definecolor{indigo}{rgb}{0.29, 0.0, 0.51}
%Pink palette
% \definecolor{p1}{RGB}{203, 167, 179}
% \definecolor{p2}{RGB}{224, 185, 216}
% \definecolor{p3}{RGB}{250, 219, 225}
% \definecolor{p4}{RGB}{247, 171, 197}
% \definecolor{p5}{RGB}{187, 161, 198}
% Grey-green-white palette
% \definecolor{p1}{RGB}{135, 136, 113}
% \definecolor{p2}{RGB}{202, 196, 175}
% \definecolor{p3}{RGB}{245, 247, 236}
% \definecolor{p4}{RGB}{217, 219, 211}
% \definecolor{p5}{RGB}{238, 239, 220}
%Gray paletter
\definecolor{p1}{gray}{0.4}
\definecolor{p2}{gray}{0.6}
\definecolor{p3}{gray}{0.98}
\definecolor{p4}{gray}{0.8}
\definecolor{p5}{gray}{0.9}

%%%%%%ToDo's%%%%%%%
% \newcommand{\ToDo}{{\bf \color{red} ToDo} }
% \newcommand{\Kasia}[1]{\todo[color=magenta!30]{{\bf Kasia:} #1}}
% \newcommand{\ikasia}[1]{\todo[inline, color=magenta!30]{{\bf Kasia:} #1}}
% \newcommand{\kasia}[1]{{\color{magenta} {#1 }}}
% \newcommand{\Michal}[1]{\todo[color=blue!30]{{\bf Micha\l:} #1}}
% \newcommand{\imichal}[1]{\todo[inline, color=blue!30]{{\bf Micha\l:} #1}}
% \newcommand{\michal}[1]{{\color{blue} {#1 }}}
% 
% \newcommand*{\red}{\textcolor{red}}

\setlength\parindent{0pt}

\setcounter{tocdepth}{1}


\belowdisplayskip=18pt plus 6pt minus 12pt \abovedisplayskip=18pt
plus 6pt minus 12pt
\parskip 8pt plus 1pt
\def\tsp{\def\baselinestretch{2.65}\large
\normalsize}


\def\dsp{\def\baselinestretch{1.35}\large
\normalsize}
%%%%This makes a double spacing. Use this with 11pt style. If you
%%%%want to use this just insert \dsp after the \begin{document}
%%%%The correct baselinestretch for double spacing is 1.37. However
%%%%you can use different parameter.

%%%%%%LITERY%%%%%%%
\newcommand{\sing}{\operatorname{sing}}
\newcommand{\HL}{\mathrm{HL}}

\def\eps{\varepsilon}
\def\vr{\varrho}
\def\Om{\Omega}
\def\om{\omega}
\def\vi{\varphi}
\def\vp{\varphi}
\def\id{{\rm id\, }}
\def\BBB{\widetilde{B}}  % metric balls

\def\nM{\mathfrak{M}}
\def\nod{{\rm Mod}}

\newcommand{\m}{\mathcal{M}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cH}{\mathcal{H}}

\def\B{{B}}
\def\C{{\mathcal C}}
\def\D{{\mathcal D}}
\def\F{{\mathcal F}}
\def\n{{\mathcal M}}
%\newcommand{\dif}{\,\mathrm{d}}

\def\N{{\mathbb N}}
\def\n{{\mathcal{M}}}
\def\n{{\mathcal N}}
\def\H{{\mathcal H}}
\def\U{{\mathcal U}}
\def\S{{\mathbb S}}
\def\I{{\mathcal I}}
\def\T{{\mathcal T}}
\newcommand{\boldg}{{\mathbf g}}

\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

\renewcommand{\div}{{\rm div}}
\newcommand{\dv}{\operatorname{div}}
\newcommand{\cJ}{\mathcal J}
\newcommand{\cB}{\mathcal B}
\newcommand{\cA}{\mathcal A}
\newcommand{\bad}{{\mathsf{Bad}}}
\newcommand{\good}{{\mathsf{Good}}}

\def\leb{{\mathcal L}}

\def\rss{{\vert_{_{_{\!\!-\!\!-\!}}}}}
%%%%%%%%%%%TWIERDZENIA%%%%%%%%%%%%
\newtheorem{theorem}{Theorem}
\newtheorem{claim}{Claim}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{exercise}[theorem]{Exercise}
%\theoremstyle{definition}
\newtheorem{remark}[theorem]{Remark}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
\newtheorem{question}[theorem]{Question}
\newtheorem{conjecture}[theorem]{Conjecture}
\newtheorem{openproblem}[theorem]{Open Problem}

%%%FUNKCJE MATEATYCZNE%%%%%%%%%
\newcommand{\loc}{\mathrm{loc}}
\def\esssup{\mathop{\rm ess\,sup\,}}
\def\essmax{\mathop{\rm ess\,max\,}}
\def\osc{\mathop{\rm osc\,}}
\def\diam{{\rm diam\,}}
\def\dist{{\rm dist\,}}
\def\divv{{\rm div\,}}
\def\rot{{\rm rot\,}}
\def\curl{{\rm curl\,}}
\def\lip{{\rm Lip\,}}
\def\rank{{\rm rank\,}}
\def\supp{{\rm supp\,}}
\def\loc{{\rm loc}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\dif}{\,\mathrm{d}}
\newcommand{\dx}{\dif x}
\newcommand{\dy}{\dif y}
\newcommand{\dz}{\dif z}
\renewcommand{\dh}{\dif\mathcal{H}}
\newcommand{\dd}{\dif}

\newcommand{\R}{\mathbb{R}}
\newcommand{\bB}{\mathbb{B}}
\newcommand{\dhn}{\dif \mathcal{H}^{n-1}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\HI}{\mathcal{H}}
\newcommand{\Z}{\mathbb{Z}}

\newcommand{\pl}{\partial}
\newcommand{\ale}{\lesssim}
\newcommand{\vrac}[1]{\| #1 \|}
\newcommand{\fracm}[1]{\frac{1}{#1}}
\newcommand{\brac}[1]{\left (#1 \right )}
\newcommand{\abs}[1]{\left |#1 \right |}
\newcommand{\Ep}{\bigwedge\nolimits}
\newcommand{\norm}[1]{\left\|{#1}\right\|}
\newcommand{\ov}[1]{\overline{#1}}
\newcommand{\la}{\left\langle}
\newcommand{\ra}{\right\rangle}

\newcommand{\Sw}{\mathcal{S}}

\newcommand{\Jac}{{\rm Jac}}

%%%%%%%%%%%%%%CALKI%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newcommand{\barint}{
\rule[.036in]{.12in}{.009in}\kern-.16in \displaystyle\int }

\newcommand{\barcal}{\mbox{$ \rule[.036in]{.11in}{.007in}\kern-.128in\int $}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\newcommand{\bbbr}{\mathbb R}
\newcommand{\bbbg}{\mathbb G}
\newcommand{\bbbh}{\mathbb H}
\newcommand{\bbbc}{\mathbb C}



\def\bbbone{{\mathchoice {\rm 1\mskip-4mu l} {\rm 1\mskip-4mu l}
{\rm 1\mskip-4.5mu l} {\rm 1\mskip-5mu l}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\def\mvint_#1{\mathchoice
          {\mathop{\vrule width 6pt height 3 pt depth -2.5pt
                  \kern -8pt \intop}\nolimits_{\kern -3pt #1}}%
%%%% P.S., 01/03/2001
% old definition had ...\nolimits_{#1}}
% \kern -3pt makes nicer distances between the integral sign
% and the domain of integration
%%%%
          {\mathop{\vrule width 5pt height 3 pt depth -2.6pt
                  \kern -6pt \intop}\nolimits_{#1}}%
          {\mathop{\vrule width 5pt height 3 pt depth -2.6pt
                  \kern -6pt \intop}\nolimits_{#1}}%
          {\mathop{\vrule width 5pt height 3 pt depth -2.6pt
                  \kern -6pt \intop}\nolimits_{#1}}}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\renewcommand{\thetheorem}{\arabic{section}.\arabic{theorem}}
\renewcommand{\theequation}{\arabic{section}.\arabic{equation}}
\renewcommand{\theparagraph}{\arabic{section}.\arabic{paragraph}}

\numberwithin{theorem}{section} \numberwithin{equation}{section}

\def\karta{\hbox{$\clubsuit$}}

\newcommand{\lap}{\Delta }
\newcommand{\aleq}{\precsim}
\newcommand{\ageq}{\succsim}
\newcommand{\aeq}{\approx}
\newcommand{\Rz}{\mathcal{R}}
\newcommand{\laps}[1]{(-\lap)^{\frac{#1}{2}}}
\newcommand{\lapv}{(-\lap)^{\frac{1}{4}}}
\newcommand{\lapms}[1]{I^{#1}}

\newcommand{\plaps}[2]{(-\lap)^{#1}_{#2}}


\newcommand{\mychi}{\raisebox{0pt}[1ex][1ex]{$\chi$}} %\chi with lower index
\newlength{\temp}

% Definition of \dashint
% Averaged integral sign
\def\Xint#1{\mathchoice
   {\XXint\displaystyle\textstyle{#1}}%
   {\XXint\textstyle\scriptstyle{#1}}%
   {\XXint\scriptstyle\scriptscriptstyle{#1}}%
   {\XXint\scriptscriptstyle\scriptscriptstyle{#1}}%
   \!\int}
\def\XXint#1#2#3{{\setbox0=\hbox{$#1{#2#3}{\int}$}
     \vcenter{\hbox{$#2#3$}}\kern-.5\wd0}}
\def\ddashint{\Xint=}
\def\dashint{\Xint-}


\let\latexchi\chi
\makeatletter
\renewcommand\chi{\@ifnextchar_\sub@chi\latexchi}
\newcommand{\sub@chi}[2]{% #1 is _, #2 is the subscript
  \@ifnextchar^{\subsup@chi{#2}}{\latexchi^{}_{#2}}%
}
\newcommand{\subsup@chi}[3]{% #1 is the subscript, #2 is ^, #3 is the superscript
  \latexchi_{#1}^{#3}%
}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%Fillin tikz%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\makeatletter
%\def\tikz@arc@opt[#1]{% over-write!
%  {%
%    \tikzset{every arc/.try,#1}%
%    \pgfkeysgetvalue{/tikz/start angle}\tikz@s
%    \pgfkeysgetvalue{/tikz/end angle}\tikz@e
%    \pgfkeysgetvalue{/tikz/delta angle}\tikz@d
%    \ifx\tikz@s\pgfutil@empty%
%      \pgfmathsetmacro\tikz@s{\tikz@e-\tikz@d}
%    \else
%      \ifx\tikz@e\pgfutil@empty%
%        \pgfmathsetmacro\tikz@e{\tikz@s+\tikz@d}
%      \fi%
%    \fi
%    \tikz@arc@moveto
%    \xdef\pgf@marshal{\noexpand%
%    \tikz@do@arc{\tikz@s}{\tikz@e}
%      {\pgfkeysvalueof{/tikz/x radius}}
%      {\pgfkeysvalueof{/tikz/y radius}}}%
%  }%
%  \pgf@marshal%
%  \tikz@arcfinal%
%}
%\let\tikz@arc@moveto\relax
%\def\tikz@arc@movetolineto#1{%
%  \def\tikz@arc@moveto{\tikz@@@parse@polar{\tikz@arc@@movetolineto#1}(\tikz@s:\pgfkeysvalueof{/tikz/x radius} and \pgfkeysvalueof{/tikz/y radius})}}
%\def\tikz@arc@@movetolineto#1#2{#1{\pgfpointadd{#2}{\tikz@last@position@saved}}}
%\tikzset{%
%  move to start/.code=\tikz@arc@movetolineto\pgfpathmoveto,%
%  line to start/.code=\tikz@arc@movetolineto\pgfpathlineto}
%\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

